Interactive Tools for Reproducible Science -- Understanding, Supporting, and Motivating Reproducible Science Practices

Reproducibility should be a cornerstone of science as it enables validation and reuse. In recent years, the scientific community and the general public became increasingly aware of the reproducibility crisis, i.e. the wide-spread inability of researchers to reproduce published work, including their own. Scientific research is increasingly focused on the creation, observation, processing, and analysis of large data volumes. On the one hand, this transition towards computational and data-intensive science poses new challenges for research reproducibility and reuse. On the other hand, increased availability and advances in computation and web technologies offer new opportunities to address the reproducibility crisis. This thesis reports on user-centered design research conducted at CERN, a key laboratory in data-intensive particle physics. In this thesis, we build a wider understanding of researchers' interactions with tools that support research documentation, preservation, and sharing. From a Human-Computer Interaction (HCI) perspective the following aspects are fundamental: (1) Characterize and map requirements and practices around research preservation and reuse. (2) Understand the wider role and impact of research data management (RDM) tools in scientific workflows. (3) Design tools and interactions that promote, motivate, and acknowledge reproducible research practices. Research reported in this thesis represents the first systematic application of HCI methods in the study and design of interactive tools for reproducible science. We advocate the unique role of HCI in supporting, motivating, and transforming reproducible research practices through the design of tools that enable effective RDM. This thesis paves new ways for interaction with RDM tools that support and motivate reproducible science.

==> chapter/00_misc/acros.tex <==
\DeclareAcronym{SUS}{short = SUS, long =  System Usability Scale}
\DeclareAcronym{6DoF}{short = 6DoF , long = six degree of freedom}
\DeclareAcronym{HCI}{short = HCI , long = Human-Computer Interaction}
\DeclareAcronym{TCT}{short = TCT , long = task completion time}
\DeclareAcronym{TLX}{short = NASA-TLX , long = NASA Task Load Index}
\DeclareAcronym{IV}{short = IV , long = independent variable}
\DeclareAcronym{DV}{short = DV , long = dependent variable}
\DeclareAcronym{LHRD}{short = LHRD, long = large high-resolution display}
\DeclareAcronym{UI}{short = UI, long = user interface}
\DeclareAcronym{GP}{short = GP, long = Gaussian Processes}
\DeclareAcronym{NN}{short = NN, long =  neural network}
\DeclareAcronym{NNR}{short = NNR, long =  neural network regression}
\DeclareAcronym{KNN}{short = KNN, long =  K-Nearest-Neighbor}
\DeclareAcronym{ReLU}{short = ReLU, long =  rectified linear unit}

==> chapter/00_misc/layout-definitions.tex <==
\definecolor{primaryColor}{HTML}{A2C2DE}
\definecolor{secondaryColor}{HTML}{E1EAF4}
\definecolor{tertiaryColor}{HTML}{cbd6e5}
%\definecolor{tertiaryColor}{HTML}{F3F7FB}
\definecolor{MyGray}{rgb}{0.86,0.87,0.88}

\definecolor{ReferenceGray}{rgb}{0.91,0.91,0.91}

\makeatletter\newenvironment{graybox}{%
   \begin{lrbox}{\@tempboxa}
   	\begin{minipage}[c]{.8\columnwidth}}{
	\end{minipage}
   \end{lrbox}%
   \colorbox{ReferenceGray}{\usebox{\@tempboxa}}
}\makeatother

\makeatletter\newenvironment{grayboxwide}{%
   \begin{lrbox}{\@tempboxa}
   	\begin{minipage}[c]{\textwidth}}{
	\end{minipage}
   \end{lrbox}%
   \colorbox{ReferenceGray}{\usebox{\@tempboxa}}
}\makeatother

\makeatletter\newenvironment{definitionbox}{%
   \begin{lrbox}{\@tempboxa}
   	\begin{minipage}[c]{.88\textwidth}	\vspace{3mm}}{
	\vspace{3mm}
	\end{minipage}
   \end{lrbox}%
   \colorbox{ReferenceGray}{\usebox{\@tempboxa}}
}\makeatother

\makeatletter\newenvironment{referencebox}{%
   \begin{lrbox}{\@tempboxa}
   	\begin{minipage}[c]{.98\textwidth}	\vspace{3mm}}{
	\vspace{3mm}
	\end{minipage}
   \end{lrbox}%
   \colorbox{ReferenceGray}{\usebox{\@tempboxa}}
}\makeatother

\newcommand{\publicationsbegin}{ 
   \begin{list}{\raise .5ex\hbox{\scriptsize$\bullet$}}
    { \setlength{\itemsep}{5pt}      \setlength{\parsep}{3pt} 
      \setlength{\topsep}{6pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.7em} } }

\newcommand{\publicationsend}{
    \end{list}  } 

\newcommand{\etal}{\mbox{et al.\,}\xspace}

==> tex/00_coauthorship.tex <==
\newcommand{\forceindent}{\leavevmode{\parindent=3em\indent}}

\specialchapter{Publications and Declaration of Co-Authorship}

All the following papers were peer-reviewed. 

\textbf{Chapter~\ref{chap:pdapps}}

Chapter~\ref{chap:pdapps} corresponds to the following workshop paper:

\begin{adjustwidth}{2cm}{}
Mohamed Khamis, Andreas Bulling, Florian Alt. \textbf{Tackling Challenges of Interactive Public Displays using Gaze.} In Adj. Proc.\,of the ACM International Joint Conference on Pervasive and Ubiquitous Computing (UbiComp 2015), pp. 763-766, 2015.
\end{adjustwidth}


i did this they did that... 

\textbf{Chapter~\ref{chap:eyepact}}

Chapter~\ref{chap:eyepact} corresponds to the following journal paper:




\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Daniel Buschek, Tobias Thieron, Florian Alt, Andreas Bulling. \textbf{EyePACT: Eye-Based Parallax Correction on Touch-Enabled Interactive Displays.} In Proc.\,ACM Interact.\,Mob.\,Wearable Ubiquitous Technol.\,(IMWUT) 1, 4, December 2017, 18 pages.
\end{adjustwidth}


i did this they did that... 


\textbf{Chapter~\ref{chap:gtmopass}}

Chapter~\ref{chap:gtmopass} corresponds to the following conference paper:

\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Regina Hasholzner, Andreas Bulling, Florian Alt. \textbf{GTmoPass: Two-factor Authentication on Public Displays Using GazeTouch passwords and Personal Mobile Devices.} In Proceedings of the 6th International Symposium on Pervasive Displays (PerDis 2017).
\end{adjustwidth}


i did this they did that... 




\textbf{Chapter~\ref{chap:eyescout}}

Chapter~\ref{chap:eyescout} corresponds to the following conference paper:

\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Axel Hoesl, Alexander Klimczak, Martin Reiss, Florian Alt, Andreas Bulling. \textbf{EyeScout: Active Eye Tracking for Position and Movement Independent Gaze Interaction with Large Public Displays.} In Proceedings of the 30th Annual ACM Symposium on User Interface Software \& Technology (UIST 2017).
\end{adjustwidth}


i did this they did that... 


\textbf{Chapter~\ref{chap:calibration}}

Section~\ref{sec:textpursuits} corresponds to the following conference paper:

\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Ozan Saltuk, Alina Hang, Katharina Stolz, Andreas Bulling, Florian Alt. \textbf{TextPursuits: Using Text for Pursuits-Based Interaction and Calibration on Public Displays.} In Proc.\,of the 2016 ACM International Joint Conference on Pervasive and Ubiquitous Computing (UbiComp 2016).
\end{adjustwidth}


i did this they did that... 


Section~\ref{sec:eyevote} corresponds to the following conference paper:

\begin{adjustwidth}{2cm}{}
    Mohamed Khamis, Ludwig Trotter, Markus Tessmann, Christina Dannhart, Andreas Bulling, Florian Alt. \textbf{EyeVote in the Wild: Do Users bother Correcting System Errors on Public Displays?} In Proc.\,of the 15th International Conference on Mobile and Ubiquitous Multimedia (MUM 2016).
\end{adjustwidth}


i did this they did that... 


% \textbf{Chapter~\ref{chap:multipleusers}}

% Chapter~\ref{chap:multipleusers} corresponds to the following conference paper:

% \begin{adjustwidth}{2cm}{}
%     TBA
% \end{adjustwidth}


\vspace{2cm}
Munich, 15.12.2017 
\hfill{\rule{4cm}{1pt}}

\hfill{Mohamed Khamis}
